Latent Translation: Crossing Modalities by Bridging Generative Models

End-to-end optimization has achieved state-of-the-art performance on many specific problems, but there is no straight-forward way to combine pretrained models for new problems. Here, we explore improving modularity by learning a post-hoc interface between two existing models to solve a new task. Specifically, we take inspiration from neural machine translation, and cast the challenging problem of cross-modal domain transfer as unsupervised translation between the latent spaces of pretrained deep generative models. By abstracting away the data representation, we demonstrate that it is possible to transfer across different modalities (e.g., image-to-audio) and even different types of generative models (e.g., VAE-to-GAN). We compare to state-of-the-art techniques and find that a straight-forward variational autoencoder is able to best bridge the two generative models through learning a shared latent space. We can further impose supervised alignment of attributes in both domains with a classifier in the shared latent space. Through qualitative and quantitative evaluations, we demonstrate that locality and semantic alignment are preserved through the transfer process, as indicated by high transfer accuracies and smooth interpolations within a class. Finally, we show this modular structure speeds up training of new interface models by several orders of magnitude by decoupling it from expensive retraining of base generative models.

==> 130 WIP Latent Transfer (ArXiV)/archiveprevious.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Domain transfer is an exciting application of deep learning.
Usually, it refers to the mapping between two domains such that the variations in one domain are reflected in the other.
Interesting existing works include transferring between two domains of different styles of image~\citep{pix2pix2016,CycleGAN2017}, 
video~\citep{wang2018vid2vid} and music~\citep{mor2018universal},
and are usually referred as ``style tranfer'' since they are operating on the style level.
These works, besides being visually appealing, 
allows intuitive control of complicated generative models that users can expect the result in the target domain is intuitively related to the source domain.
Furthermore, learning transformation is easier than learning full generative model.

Despite being interesting, this line of works in domain transfer has several limitations.
The first limitation is that, it requires that two domains where the model transfers should be closely related (e.g. image-to-image or video-to-video).
The model also transfer local properties like texture and coloring instead of high level semantics,
for example, directly applying CycleGAN or its variants to images of not-so-close domains leads to distorted or wired results~\citep{li2018unsupervised}.
Even the task of transferring between texture styles are not done principledly,
as shown in  \citet{chu2017cyclegan} that CycleGAN hides texture on source domain in the high frequency part of target domain and
generate the visible texture (low-frequency part) regardless of the source.

The second limitation is data efficiency: Some techniques in the line of style transfer need lots of paired data.
For example, vid2vid~\citep{wang2018vid2vid} requires frame-by-frame pairs as the training data.
Usually one side of the domains essentially a dense feature extraction of the other, 
for example in vid2vid's case one side is the segmentation of the other as image.
This makes the transfer model learn a inverse feature extraction,
and is usually infeasible for different domains, such as image-to-audio scenario.

We investigate the prior limitations and propose a general-purposed domain transfer model that,
instead of transfer between data space,
bridge between the latent spaces of two pre-trained generative models on two domains respectively.
The fact of transferring between latent spaces rather than data space enables transfer across modalities, such as between audio and images, as long as we have generative models on them.
Moreover the transfer can happen between generative models of different nature, like between VAE and GAN.
Finally since the domain-specific structures are captured by these pre-trained generative models which only need to be trained once,
our approach thus can more efficiently leveraged the paired data, increasing the sample and computational efficiency.

\WritingSketch{
Our contribution is...
The rest of the paper is organized as follow:... 
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Background}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth,trim={0 0 0 0},clip]{figure/Fig-Overview2.pdf}
\caption{The overall structure of our method. 
As shown in this figure,
our method (show in dark) works, through the use of a shared latent space ($Z'$), bridges between the latent spaces ($Z_1, Z_2$) of two pre-trained generative models (shown in blue) in the dataspace ($X_1, X_2$).
One the left we show the general architecture, which on the right 
}
\label{fig:overall}
\end{figure}


% Generative Model. VAE and GAN --- how they work, how they are optimized, how the latent space and data space are related.

Generative model with latent space are usually done in a fashion that transfer a simple, tractable distribution $p(z)$
into the approximation of population distribution $p^*(x)$.
This transfer is usually completed through the use of deep neural network based decoder.
We denote the space $Z$ that $z$ is sampled from  \emph{latent space} while the population space $X$ \emph{data space}.
Such model includes VAE~\citep{kingma2013auto} and GAN~\citep{goodfellow2014generative}.
GANs are trained with an accompany classifier that attempts to distinguish between samples from decoder and from true dataset $X*$.
VAEs, in the contrast, are trained with a encoder distribution $q(z|x)$ as a apparoximation to the posterior $p(z|x)$ using 
variational approximation through the use of evidence lower bound (ELBO):
\[ 
\mathcal{L}^{\mathrm{ELBO}} = \E_{x\sim p(x), z\sim q(z|x)} \left[ \log \pi (x ; g(z)) \right] - \mathcal{D}_{\mathrm{KL}} \left( q(z|x) || p(z) \right)  % fix || in D
\]
where $\pi$, defined as $p(x|z)$, is a likelihood function measures the similarity of $x$ and decoded result $g(z)$.


%Existing transfer:
%1. How they work? usually between data space. 
%2. One Issue : Between data space = locality transfer. texture level.
%3. Another: data efficiency.

One the other hand, the domain transfer 
that enables transfer between images, audio and video, % TODO: cite
intuitively refers to mapping between two domains 
where the variations in one domain should be reflected in the other.
Formally, for samples in one domain ($x_1 \sim X_1$), the transfer shall produces samples in other one ($x_2 \sim X_2$) though the (possibly implicit) estimation $p(x_2| x_1)$.
Although these works are exiting and visually appalling, 
recently is has been proposed that several limitations exist:
\cite{chu2017cyclegan} suggests that image transfer does only local, texture level transfer, 
and to make things worse, even this transfer is not done properly, 
such that the model usually learns to hide the information of original texture and impaint the texture in the target domain,
instead of meaningfully transfer the texture to reflect the variation in the original domain's texture.
Furthermore, Some techniques in the line of style transfer need lots of paired data.
For example, \cite{wang2018vid2vid} requires frame-by-frame pairs as the training data.
this is because one domain is usually the feature extracted from the other (e.g. the segmentation of a photo-realistic image), 
and learning an inverse feature extraction requires dense supervision,
which is at best requiring lots of paired training data and at worst not feasible for domains that are drastically different
such as images and audio.


% Our method is a combination of both
Towards mitigate the issues in domain transfer methods,
from a different point of view,
we propose to leverage the latent space to transfer between instances from two domains $\left( x_1\sim X_1, x_2\sim X_2 \right)$.
We first prepare two \emph{independent, pre-trained} generative models on two domains,
which enables the encoding of data domain to the latent space (e.g.~ $Z_1$ and $Z_2$) in form of $q(z_1|x_1)$ and $q(z_2|x_2)$
as well as the decoding via $g(z_1)$ and $g(z_2)$.
These pre-trained models are usually explicit generative models such as VAEs to enable the encoding and are trained with good reconstruction performance in mind, but it could also be implicit generative models such as GAN where $q(z|x)$ is approximated by sampling from $p(z)$ and selectes $z$s whose associated generate result $g(z)$ is given high confidence by an auxiliary classifier on $X$.
Then we train two VAEs with shared latent space $Z'$ that models $Z_1$ and $Z_2$, 
the latent spaces of aforementioned generative models respectively. 
One VAE enables estimating the $q(z'|z_1)$ and $p(z_1|z')$ though encoder and decoder combination,
while the aother VAE does the same for  $q(z'|z_2)$ and $p(z_2|z')$.
Due to the introducting the shared latent space $Z'$,
also domain transfer $z_2\sim p(z_2|z') p(z'|z_1)$ and joint sampling $z'\sim p(z'), (z_1, z_2) \sim p(z_1, z_2 | z') = p(z_1|z') p(z_2|z')$ are enabled.

The overall structure of our approach is shown in Figure~\ref{fig:overall}, 
and the details go though Section~\ref{sec:overall-architecture}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Overall Architecture}
\label{sec:overall-architecture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\WritingSketch{
Overall architecture.
Use two VAEs with shared space Z’ to model two spaces Z1 and Z2 of pretrained model.
Enables transfer and joint sampling.
Enables semi supervised  training. (loss term vs. components)
}

\WritingSketch{
What is the position of this architecture? How it is related to pre-trained model? How transfer and joint sampling is done?
}

\WritingSketch{
How semi supervised training is done?
leverage unsupervised alignment of the latent spaces to increase data-efficiency .
data: $z_1 \sim q(z1|x1)p(x1), z2 \sim q(z2|x2)p(x2)$.
reducing the required number of supervised data pairs.
data: $ (z_1, z_2) \sim     q(z_1|x_1) q(z_2|x_2) p(x_1, x_2)$.
}

\WritingSketch{
What is the loss funciton? loss function? Elaborate each component of loss. 
}




\begin{figure}[t!]
\centering
\includegraphics[width=\textwidth,trim={0 0 0 0},clip]{figure/Fig-Arch.pdf}
\caption{The architecture of our network.
}
\label{fig:arch}
\end{figure}

\WritingSketch{
 what is the concrete architecture? What is ours? What is the pretrained
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Network Architecture and training}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\WritingSketch{
Concrete architecture...
Encoders and Decoders: Fully-connected
ReLU stacks with a “Gated Mixing Layer”.
Gated Mixing Layer helps optimization by starting with a good initialization.
}


\WritingSketch{
Pretrain's model's structure
}


\WritingSketch{
how to prepare data? (sepecially for GAN)
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Qualitative Experiments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We conduct qualitative experiments in several settings to reveal the performance and properties of our proposed approach.
We consider following three domains: 
(a) MNIST, which is images of hand-written digits of 10 classes from ``0'' to ``9'', 
(b) Fashion MNIST, which is images of fashion related objects such as shoes, t-shirts, categorized into 10 classes, and
(c) SC09, which is the audio record of human saying digits from ``0'' to ``'9''.
For (a) and (b) we prepare VAE with MLP encoder and decoder as the pre-trained generative model,
for (c) we use WaveGAN~\cite{donahue2018synthesizing}, an GAN on SC09 dataset for the purpose.


We set three scenarios of transfer.
(1) MNIST $\leftrightarrow$ MNIST, which servers as a proof of concept, 
(2) MNIST $\leftrightarrow$ Fashion MNIST, which transfers between images of a class of digit and images of a class of fashion object, and
(3) MNIST $\leftrightarrow$ SC09, which transfers between images of a class of digit and audio of the same class of digits.
The paired alignment data is collected in the following way:
For (1) a digit classes should go to the same digit class in the target domain ;
for (2) we specify a global mapping between 10 digit classes and 10 fashion object classes, ;
and for (3) the image of one digit class is matched with same digit class' audio version, which means an image of hand-written ``0'' should match an (arbitrary) audio version of ``0'' spoken by human.
We would like to emphasis that we only use \emph{label level} alignment, which means in the training we draw randomly $x_1, x_2$ with equivalent classes, This approach is aligned with our argument that only high, semantic level alignment is used, instead of local level reverse feature extraction.

\WritingSketch{
 what is the concrete architecture? What is ours? What is the pretrained
}




\WritingSketch{We show the transfer setting (1) and (2) in Figure~\ref{fig:transfer1}. Discuss.}

\begin{figure}[h!]
\centering
\includegraphics[width=\textwidth,trim={0 2.5cm 0 2.5cm},clip]{figure/Fig-Transfer1.pdf}
\caption{Transfer between MNIST $\leftrightarrow$ MNIST and MNIST $\leftrightarrow$ Fashion MNIST respectively}
\label{fig:transfer1}
\end{figure}

\WritingSketch{We show the transfer setting (1) and (2) in Figure~\ref{fig:transfer2}. Discuss}

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth,trim={0 2.5cm 0 2.5cm},clip]{figure/Fig-Transfer2.pdf}
\caption{Transfer between MNIST and SC09.}
\label{fig:transfer2}
\end{figure}


\WritingSketch{
We show the interpolation in Figure~\cite{inter1}
}

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth,trim={0 5cm 0 0},clip]{figure/Fig-inter1.pdf}
\caption{Interpolations of two sets of settings, MNIST $\leftrightarrow$ MNIST (upper) and MNIST $\leftrightarrow$ Fashion MNIST (lower).\\
In each setting,
Row 1 is the interpolation between label 0,1,7,8,3 from source domain’s VAE only;
Row 2 is the ransfer latent space of Row 1 to Target domain;
Row 3 is the interpolation between label 0,1,7,8,3 (or 0,1,7,8,3 -th labels e.g.~ T-shirt / Trouser / Sneaker / Bag / Dress,  in Fashion MNIST's case)from target domain’s VAE only.
}
\label{fig:inter1}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Quantitative Experiments}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\WritingSketch{
Measured by a trained classifier.
Accuracy = portion of instances that x1 and x2 have the same class.
}

\WritingSketch{
Protocol:
Sample chain: x1 $\to$ z1 $\to$ z’ $\to$ z2$\to$x2
Note for WaveGAN: Since GAN has not encoder, we create the paired data for WaveGAN transfer using a pre-trained classifier.
}


\begin{table}[h]
  \center
  \begin{tabular}{l | l  l  l }
  \toprule
   Transfer Direction &
Transfer Accuracy &
Reconstruction Accuracy* &
Relative\\
  \midrule
   MNIST $\to$ MNIST &  .9728 & .9831 & .9895 \\
 MNIST $\to$ Fashion MNIST &
.9469 &
.9825 &
.9637 \\
SC09 (WaveGAN) $\to$  MNIST &
.9557 &
.9696** &
.9857 \\
MNIST $\to$  C09 &
.4683 &
.9696** &
.4830 \\

  \bottomrule
  \end{tabular}
  \caption{Transfer Accuracy.\\
  * The reconstruction accuracy is the upper threshold given the current evaluation protocol.\\
  ** Latent training points for GAN were selected for generating data with peaked classification distributions.
  }
  \label{tbl:transfer-accuracy}
\end{table}



\WritingSketch{
Accuracy = portion of instances that x1 and x2 have the same class.
Protocol:Sample chain: $x1 \to z1 \to z’ \to z2 \to x2$
Note for WaveGAN: Since GAN has not encoder, we create the paired data for WaveGAN transfer using a pre-trained classifier.
}

\subsection{joint sample accuarcy}


\WritingSketch{
Protocol:
Same as Transfer Accuracy, expect that sample chain is: $ z’ \sim p(z’), z’ \to z1 \to x1, z’ \to z2 \to x2$
}

\subsection{Sample efficiency}

\begin{table}[h]
  \center
  \begin{tabular}{l | l  l  l }
  \toprule
 Total \# Paired data &
\# Paired data per label*&
Transfer Accuracy\\
\midrule
10&
1&
.4435\\
50&
5&
.5944\\
100&
10&
.6450\\
500&
50&
.812\\
1000&
100&
.8668\\
5000&
500&
.9558\\
60000
(All MNIST train data)&
\~ 6000**&
.9728\\
  \bottomrule
  \end{tabular}
  \caption{Sample Efficiency, tested on MNIST $\leftrightarrow$ MNIST Transfer\\.
* Since MNIST has 10 labels, the number of paired data for one label is this total number of paired data divided by 10.\\
** Note that MNIST is not perfectly label-balanced. 
  }
  \label{tbl:sample-efficiency}
\end{table}


\WritingSketch{See Figure~\ref{tbl:sample-efficiency}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{discussion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\WritingSketch{
training time.
efficiency.
}





\section{Related Works}

QVAE~\citep{van2017neural}

Everyone dance now~\cite{chan2018everybody}


\section{Conclusion}


%%%%%%%%%%%%%%%%%%%%%%%%%%
% Typesetting cheatsheet %
%%%%%%%%%%%%%%%%%%%%%%%%%%
%  - Citation: ~\citet or \citep. Not \cite
%
%  - Figure:
%
%      \begin{figure}[h]
%      \begin{center}
%      %\framebox[4.0in]{$\;$}
%      \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%      \end{center}
%      \caption{Sample figure caption.}
%      \end{figure}
%
%   - Table:
%
%      \begin{table}[t]
%      \caption{Sample table title}
%      \label{sample-table}
%      \begin{center}
%      \begin{tabular}{ll}
%      \multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
%      \\ \hline \\
%      Dendrite         &Input terminal \\
%      Axon             &Output terminal \\
%      Soma             &Cell body (contains cell nucleus) \\
%      \end{tabular}
%      \end{center}
%      \end{table}
%
%  - Included Figure:
%
%      \usepackage[pdftex]{graphicx} 
%      \includegraphics[width=0.8\linewidth]{myfile.pdf}
%
%  - Math symbols
%      (see symbols below)

\begin{comment}

\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}

\end{comment}




==> 130 WIP Latent Transfer (ArXiV)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> archiveprevious.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Domain transfer is an exciting application of deep learning.
Usually, it refers to the mapping between two domains such that the variations in one domain are reflected in the other.
Interesting existing works include transferring between two domains of different styles of image~\citep{pix2pix2016,CycleGAN2017}, 
video~\citep{wang2018vid2vid} and music~\citep{mor2018universal},
and are usually referred as ``style tranfer'' since they are operating on the style level.
These works, besides being visually appealing, 
allows intuitive control of complicated generative models that users can expect the result in the target domain is intuitively related to the source domain.
Furthermore, learning transformation is easier than learning full generative model.

Despite being interesting, this line of works in domain transfer has several limitations.
The first limitation is that, it requires that two domains where the model transfers should be closely related (e.g. image-to-image or video-to-video).
The model also transfer local properties like texture and coloring instead of high level semantics,
for example, directly applying CycleGAN or its variants to images of not-so-close domains leads to distorted or wired results~\citep{li2018unsupervised}.
Even the task of transferring between texture styles are not done principledly,
as shown in  \citet{chu2017cyclegan} that CycleGAN hides texture on source domain in the high frequency part of target domain and
generate the visible texture (low-frequency part) regardless of the source.

The second limitation is data efficiency: Some techniques in the line of style transfer need lots of paired data.
For example, vid2vid~\citep{wang2018vid2vid} requires frame-by-frame pairs as the training data.
Usually one side of the domains essentially a dense feature extraction of the other, 
for example in vid2vid's case one side is the segmentation of the other as image.
This makes the transfer model learn a inverse feature extraction,
and is usually infeasible for different domains, such as image-to-audio scenario.

We investigate the prior limitations and propose a general-purposed domain transfer model that,
instead of transfer between data space,
bridge between the latent spaces of two pre-trained generative models on two domains respectively.
The fact of transferring between latent spaces rather than data space enables transfer across modalities, such as between audio and images, as long as we have generative models on them.
Moreover the transfer can happen between generative models of different nature, like between VAE and GAN.
Finally since the domain-specific structures are captured by these pre-trained generative models which only need to be trained once,
our approach thus can more efficiently leveraged the paired data, increasing the sample and computational efficiency.

\WritingSketch{
Our contribution is...
The rest of the paper is organized as follow:... 
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Background}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth,trim={0 0 0 0},clip]{figure/Fig-Overview2.pdf}
\caption{The overall structure of our method. 
As shown in this figure,
our method (show in dark) works, through the use of a shared latent space ($Z'$), bridges between the latent spaces ($Z_1, Z_2$) of two pre-trained generative models (shown in blue) in the dataspace ($X_1, X_2$).
One the left we show the general architecture, which on the right 
}
\label{fig:overall}
\end{figure}


% Generative Model. VAE and GAN --- how they work, how they are optimized, how the latent space and data space are related.

Generative model with latent space are usually done in a fashion that transfer a simple, tractable distribution $p(z)$
into the approximation of population distribution $p^*(x)$.
This transfer is usually completed through the use of deep neural network based decoder.
We denote the space $Z$ that $z$ is sampled from  \emph{latent space} while the population space $X$ \emph{data space}.
Such model includes VAE~\citep{kingma2013auto} and GAN~\citep{goodfellow2014generative}.
GANs are trained with an accompany classifier that attempts to distinguish between samples from decoder and from true dataset $X*$.
VAEs, in the contrast, are trained with a encoder distribution $q(z|x)$ as a apparoximation to the posterior $p(z|x)$ using 
variational approximation through the use of evidence lower bound (ELBO):
\[ 
\mathcal{L}^{\mathrm{ELBO}} = \E_{x\sim p(x), z\sim q(z|x)} \left[ \log \pi (x ; g(z)) \right] - \mathcal{D}_{\mathrm{KL}} \left( q(z|x) || p(z) \right)  % fix || in D
\]
where $\pi$, defined as $p(x|z)$, is a likelihood function measures the similarity of $x$ and decoded result $g(z)$.


%Existing transfer:
%1. How they work? usually between data space. 
%2. One Issue : Between data space = locality transfer. texture level.
%3. Another: data efficiency.

One the other hand, the domain transfer 
that enables transfer between images, audio and video, % TODO: cite
intuitively refers to mapping between two domains 
where the variations in one domain should be reflected in the other.
Formally, for samples in one domain ($x_1 \sim X_1$), the transfer shall produces samples in other one ($x_2 \sim X_2$) though the (possibly implicit) estimation $p(x_2| x_1)$.
Although these works are exiting and visually appalling, 
recently is has been proposed that several limitations exist:
\cite{chu2017cyclegan} suggests that image transfer does only local, texture level transfer, 
and to make things worse, even this transfer is not done properly, 
such that the model usually learns to hide the information of original texture and impaint the texture in the target domain,
instead of meaningfully transfer the texture to reflect the variation in the original domain's texture.
Furthermore, Some techniques in the line of style transfer need lots of paired data.
For example, \cite{wang2018vid2vid} requires frame-by-frame pairs as the training data.
this is because one domain is usually the feature extracted from the other (e.g. the segmentation of a photo-realistic image), 
and learning an inverse feature extraction requires dense supervision,
which is at best requiring lots of paired training data and at worst not feasible for domains that are drastically different
such as images and audio.


% Our method is a combination of both
Towards mitigate the issues in domain transfer methods,
from a different point of view,
we propose to leverage the latent space to transfer between instances from two domains $\left( x_1\sim X_1, x_2\sim X_2 \right)$.
We first prepare two \emph{independent, pre-trained} generative models on two domains,
which enables the encoding of data domain to the latent space (e.g.~ $Z_1$ and $Z_2$) in form of $q(z_1|x_1)$ and $q(z_2|x_2)$
as well as the decoding via $g(z_1)$ and $g(z_2)$.
These pre-trained models are usually explicit generative models such as VAEs to enable the encoding and are trained with good reconstruction performance in mind, but it could also be implicit generative models such as GAN where $q(z|x)$ is approximated by sampling from $p(z)$ and selectes $z$s whose associated generate result $g(z)$ is given high confidence by an auxiliary classifier on $X$.
Then we train two VAEs with shared latent space $Z'$ that models $Z_1$ and $Z_2$, 
the latent spaces of aforementioned generative models respectively. 
One VAE enables estimating the $q(z'|z_1)$ and $p(z_1|z')$ though encoder and decoder combination,
while the aother VAE does the same for  $q(z'|z_2)$ and $p(z_2|z')$.
Due to the introducting the shared latent space $Z'$,
also domain transfer $z_2\sim p(z_2|z') p(z'|z_1)$ and joint sampling $z'\sim p(z'), (z_1, z_2) \sim p(z_1, z_2 | z') = p(z_1|z') p(z_2|z')$ are enabled.

The overall structure of our approach is shown in Figure~\ref{fig:overall}, 
and the details go though Section~\ref{sec:overall-architecture}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Overall Architecture}
\label{sec:overall-architecture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\WritingSketch{
Overall architecture.
Use two VAEs with shared space Z’ to model two spaces Z1 and Z2 of pretrained model.
Enables transfer and joint sampling.
Enables semi supervised  training. (loss term vs. components)
}

\WritingSketch{
What is the position of this architecture? How it is related to pre-trained model? How transfer and joint sampling is done?
}

\WritingSketch{
How semi supervised training is done?
leverage unsupervised alignment of the latent spaces to increase data-efficiency .
data: $z_1 \sim q(z1|x1)p(x1), z2 \sim q(z2|x2)p(x2)$.
reducing the required number of supervised data pairs.
data: $ (z_1, z_2) \sim     q(z_1|x_1) q(z_2|x_2) p(x_1, x_2)$.
}

\WritingSketch{
What is the loss funciton? loss function? Elaborate each component of loss. 
}




\begin{figure}[t!]
\centering
\includegraphics[width=\textwidth,trim={0 0 0 0},clip]{figure/Fig-Arch.pdf}
\caption{The architecture of our network.
}
\label{fig:arch}
\end{figure}

\WritingSketch{
 what is the concrete architecture? What is ours? What is the pretrained
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Network Architecture and training}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\WritingSketch{
Concrete architecture...
Encoders and Decoders: Fully-connected
ReLU stacks with a “Gated Mixing Layer”.
Gated Mixing Layer helps optimization by starting with a good initialization.
}


\WritingSketch{
Pretrain's model's structure
}


\WritingSketch{
how to prepare data? (sepecially for GAN)
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Qualitative Experiments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We conduct qualitative experiments in several settings to reveal the performance and properties of our proposed approach.
We consider following three domains: 
(a) MNIST, which is images of hand-written digits of 10 classes from ``0'' to ``9'', 
(b) Fashion MNIST, which is images of fashion related objects such as shoes, t-shirts, categorized into 10 classes, and
(c) SC09, which is the audio record of human saying digits from ``0'' to ``'9''.
For (a) and (b) we prepare VAE with MLP encoder and decoder as the pre-trained generative model,
for (c) we use WaveGAN~\cite{donahue2018synthesizing}, an GAN on SC09 dataset for the purpose.


We set three scenarios of transfer.
(1) MNIST $\leftrightarrow$ MNIST, which servers as a proof of concept, 
(2) MNIST $\leftrightarrow$ Fashion MNIST, which transfers between images of a class of digit and images of a class of fashion object, and
(3) MNIST $\leftrightarrow$ SC09, which transfers between images of a class of digit and audio of the same class of digits.
The paired alignment data is collected in the following way:
For (1) a digit classes should go to the same digit class in the target domain ;
for (2) we specify a global mapping between 10 digit classes and 10 fashion object classes, ;
and for (3) the image of one digit class is matched with same digit class' audio version, which means an image of hand-written ``0'' should match an (arbitrary) audio version of ``0'' spoken by human.
We would like to emphasis that we only use \emph{label level} alignment, which means in the training we draw randomly $x_1, x_2$ with equivalent classes, This approach is aligned with our argument that only high, semantic level alignment is used, instead of local level reverse feature extraction.

\WritingSketch{
 what is the concrete architecture? What is ours? What is the pretrained
}




\WritingSketch{We show the transfer setting (1) and (2) in Figure~\ref{fig:transfer1}. Discuss.}

\begin{figure}[h!]
\centering
\includegraphics[width=\textwidth,trim={0 2.5cm 0 2.5cm},clip]{figure/Fig-Transfer1.pdf}
\caption{Transfer between MNIST $\leftrightarrow$ MNIST and MNIST $\leftrightarrow$ Fashion MNIST respectively}
\label{fig:transfer1}
\end{figure}

\WritingSketch{We show the transfer setting (1) and (2) in Figure~\ref{fig:transfer2}. Discuss}

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth,trim={0 2.5cm 0 2.5cm},clip]{figure/Fig-Transfer2.pdf}
\caption{Transfer between MNIST and SC09.}
\label{fig:transfer2}
\end{figure}


\WritingSketch{
We show the interpolation in Figure~\cite{inter1}
}

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth,trim={0 5cm 0 0},clip]{figure/Fig-inter1.pdf}
\caption{Interpolations of two sets of settings, MNIST $\leftrightarrow$ MNIST (upper) and MNIST $\leftrightarrow$ Fashion MNIST (lower).\\
In each setting,
Row 1 is the interpolation between label 0,1,7,8,3 from source domain’s VAE only;
Row 2 is the ransfer latent space of Row 1 to Target domain;
Row 3 is the interpolation between label 0,1,7,8,3 (or 0,1,7,8,3 -th labels e.g.~ T-shirt / Trouser / Sneaker / Bag / Dress,  in Fashion MNIST's case)from target domain’s VAE only.
}
\label{fig:inter1}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Quantitative Experiments}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\WritingSketch{
Measured by a trained classifier.
Accuracy = portion of instances that x1 and x2 have the same class.
}

\WritingSketch{
Protocol:
Sample chain: x1 $\to$ z1 $\to$ z’ $\to$ z2$\to$x2
Note for WaveGAN: Since GAN has not encoder, we create the paired data for WaveGAN transfer using a pre-trained classifier.
}


\begin{table}[h]
  \center
  \begin{tabular}{l | l  l  l }
  \toprule
   Transfer Direction &
Transfer Accuracy &
Reconstruction Accuracy* &
Relative\\
  \midrule
   MNIST $\to$ MNIST &  .9728 & .9831 & .9895 \\
 MNIST $\to$ Fashion MNIST &
.9469 &
.9825 &
.9637 \\
SC09 (WaveGAN) $\to$  MNIST &
.9557 &
.9696** &
.9857 \\
MNIST $\to$  C09 &
.4683 &
.9696** &
.4830 \\

  \bottomrule
  \end{tabular}
  \caption{Transfer Accuracy.\\
  * The reconstruction accuracy is the upper threshold given the current evaluation protocol.\\
  ** Latent training points for GAN were selected for generating data with peaked classification distributions.
  }
  \label{tbl:transfer-accuracy}
\end{table}



\WritingSketch{
Accuracy = portion of instances that x1 and x2 have the same class.
Protocol:Sample chain: $x1 \to z1 \to z’ \to z2 \to x2$
Note for WaveGAN: Since GAN has not encoder, we create the paired data for WaveGAN transfer using a pre-trained classifier.
}

\subsection{joint sample accuarcy}


\WritingSketch{
Protocol:
Same as Transfer Accuracy, expect that sample chain is: $ z’ \sim p(z’), z’ \to z1 \to x1, z’ \to z2 \to x2$
}

\subsection{Sample efficiency}

\begin{table}[h]
  \center
  \begin{tabular}{l | l  l  l }
  \toprule
 Total \# Paired data &
\# Paired data per label*&
Transfer Accuracy\\
\midrule
10&
1&
.4435\\
50&
5&
.5944\\
100&
10&
.6450\\
500&
50&
.812\\
1000&
100&
.8668\\
5000&
500&
.9558\\
60000
(All MNIST train data)&
\~ 6000**&
.9728\\
  \bottomrule
  \end{tabular}
  \caption{Sample Efficiency, tested on MNIST $\leftrightarrow$ MNIST Transfer\\.
* Since MNIST has 10 labels, the number of paired data for one label is this total number of paired data divided by 10.\\
** Note that MNIST is not perfectly label-balanced. 
  }
  \label{tbl:sample-efficiency}
\end{table}


\WritingSketch{See Figure~\ref{tbl:sample-efficiency}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{discussion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\WritingSketch{
training time.
efficiency.
}





\section{Related Works}

QVAE~\citep{van2017neural}

Everyone dance now~\cite{chan2018everybody}


\section{Conclusion}


%%%%%%%%%%%%%%%%%%%%%%%%%%
% Typesetting cheatsheet %
%%%%%%%%%%%%%%%%%%%%%%%%%%
%  - Citation: ~\citet or \citep. Not \cite
%
%  - Figure:
%
%      \begin{figure}[h]
%      \begin{center}
%      %\framebox[4.0in]{$\;$}
%      \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%      \end{center}
%      \caption{Sample figure caption.}
%      \end{figure}
%
%   - Table:
%
%      \begin{table}[t]
%      \caption{Sample table title}
%      \label{sample-table}
%      \begin{center}
%      \begin{tabular}{ll}
%      \multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
%      \\ \hline \\
%      Dendrite         &Input terminal \\
%      Axon             &Output terminal \\
%      Soma             &Cell body (contains cell nucleus) \\
%      \end{tabular}
%      \end{center}
%      \end{table}
%
%  - Included Figure:
%
%      \usepackage[pdftex]{graphicx} 
%      \includegraphics[width=0.8\linewidth]{myfile.pdf}
%
%  - Math symbols
%      (see symbols below)

\begin{comment}

\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}

\end{comment}



